Design of Novel Analog Compute Paradigms with Ark

Previous efforts on reconfigurable analog circuits mostly focused on specialized analog circuits, produced through careful co-design, or on highly reconfigurable, but relatively resource inefficient, accelerators that implement analog compute paradigms. This work deals with an intermediate point in the design space: Specialized reconfigurable circuits for analog compute paradigms. This class of circuits requires new methodologies for performing co-design, as prior techniques are typically highly specialized to conventional circuit classes (e.g., filters, ADCs). In this context, we present Ark, a programming language for describing analog compute paradigms. Ark enables progressive incorporation of analog behaviors into computations, and deploys a validator and dynamical system compiler for verifying and simulating computations. We use Ark to codify the design space for three different exemplary circuit design problems, and demonstrate that Ark helps exploring design trade-offs and evaluating the impact of nonidealities to the computation.

==> gen-specs/func-example-br-tln-Em-hwtln-lang.tex <==
{\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\footnotesize,fontseries=b]
\textcolor{black}{\textbf{func}} \textcolor{deepred}{br-tln-Em} \textcolor{black}{\textbf{(}}\textcolor{deepred}{sw}\textcolor{black}{\textbf{:}} \textcolor{black}{\textbf{int}}\textcolor{black}{\textbf{[}}\textcolor{deepred}{0}\textcolor{black}{\textbf{,}} \textcolor{deepred}{1}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{)}}
\textcolor{black}{\textbf{uses}} \textcolor{deepred}{hwtln-lang}\textcolor{black}{\textbf{\{}}
  ...
  \textcolor{black}{\textbf{node}} \textcolor{deepred}{n\_v10}\textcolor{black}{\textbf{:}} \textcolor{deepred}{V}
  \textcolor{black}{\textbf{node}} \textcolor{deepred}{n\_i11}\textcolor{black}{\textbf{:}} \textcolor{deepred}{I}
  \textcolor{black}{\textbf{node}} \textcolor{deepred}{n\_ibr}\textcolor{black}{\textbf{:}} \textcolor{deepred}{I}
  \textcolor{black}{\textbf{edge<}}\textcolor{deepred}{n\_v10}\textcolor{black}{\textbf{,}} \textcolor{deepred}{n\_i11}\textcolor{black}{\textbf{>}} \textcolor{deepred}{e\_10\_11}\textcolor{black}{\textbf{:}} \textcolor{deepred}{Em}
  \textcolor{black}{\textbf{edge<}}\textcolor{deepred}{n\_i11}\textcolor{black}{\textbf{,}} \textcolor{deepred}{n\_ibr}\textcolor{black}{\textbf{>}} \textcolor{deepred}{e\_10\_br}\textcolor{black}{\textbf{:}} \textcolor{deepred}{Em}\textcolor{deepred}{\_sw}
  \textcolor{black}{\textbf{set-switch}} \textcolor{deepred}{n\_ibr} \textcolor{black}{\textbf{when}} \textcolor{green}{sw==1}
  ...
\textcolor{black}{\textbf{\}}}
\end{Verbatim}
}

==> gen-specs/func-example-br-tln-Nm-hwtln-lang.tex <==
{\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\footnotesize,fontseries=b]
\textcolor{black}{\textbf{func}} \textcolor{deepred}{br-tln-Nm} \textcolor{black}{\textbf{(}}\textcolor{deepred}{sw}\textcolor{black}{\textbf{:}} \textcolor{black}{\textbf{int}}\textcolor{black}{\textbf{[}}\textcolor{deepred}{0}\textcolor{black}{\textbf{,}} \textcolor{deepred}{1}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{)}}
\textcolor{black}{\textbf{uses}} \textcolor{deepred}{hwtln-lang}\textcolor{black}{\textbf{\{}}
  ...
  \textcolor{black}{\textbf{node}} \textcolor{deepred}{n\_v10}\textcolor{black}{\textbf{:}} \textcolor{deepred}{Vm}
  \textcolor{black}{\textbf{node}} \textcolor{deepred}{n\_i11}\textcolor{black}{\textbf{:}} \textcolor{deepred}{Im}
  \textcolor{black}{\textbf{node}} \textcolor{deepred}{n\_ibr}\textcolor{black}{\textbf{:}} \textcolor{deepred}{Im}
  \textcolor{black}{\textbf{edge<}}\textcolor{deepred}{n\_v10}\textcolor{black}{\textbf{,}} \textcolor{deepred}{n\_i11}\textcolor{black}{\textbf{>}} \textcolor{deepred}{e\_10\_11}\textcolor{black}{\textbf{:}} \textcolor{deepred}{E}
  \textcolor{black}{\textbf{edge<}}\textcolor{deepred}{n\_i11}\textcolor{black}{\textbf{,}} \textcolor{deepred}{n\_ibr}\textcolor{black}{\textbf{>}} \textcolor{deepred}{e\_10\_br}\textcolor{black}{\textbf{:}} \textcolor{deepred}{E}\textcolor{deepred}{\_sw}
  \textcolor{black}{\textbf{set-switch}} \textcolor{deepred}{n\_ibr} \textcolor{black}{\textbf{when}} \textcolor{green}{sw==1}
  ...
\textcolor{black}{\textbf{\}}}
\end{Verbatim}
}

==> gen-specs/func-example-br-tln-tln-lang.tex <==
{\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\footnotesize,fontseries=b]
\textcolor{black}{\textbf{func}} \textcolor{deepred}{br-tln} \textcolor{black}{\textbf{(}}\textcolor{deepred}{sw}\textcolor{black}{\textbf{:}} \textcolor{black}{\textbf{int}}\textcolor{black}{\textbf{[}}\textcolor{deepred}{0}\textcolor{black}{\textbf{,}} \textcolor{deepred}{1}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{)}}
\textcolor{black}{\textbf{uses}} \textcolor{deepred}{tln-lang}\textcolor{black}{\textbf{\{}}
  ...
  \textcolor{black}{\textbf{node}} \textcolor{deepred}{n\_v10}\textcolor{black}{\textbf{:}} \textcolor{deepred}{V}
  \textcolor{black}{\textbf{node}} \textcolor{deepred}{n\_i11}\textcolor{black}{\textbf{:}} \textcolor{deepred}{I}
  \textcolor{black}{\textbf{node}} \textcolor{deepred}{n\_ibr}\textcolor{black}{\textbf{:}} \textcolor{deepred}{I}
  \textcolor{black}{\textbf{edge<}}\textcolor{deepred}{n\_v10}\textcolor{black}{\textbf{,}} \textcolor{deepred}{n\_i11}\textcolor{black}{\textbf{>}} \textcolor{deepred}{e\_10\_11}\textcolor{black}{\textbf{:}} \textcolor{deepred}{E}
  \textcolor{black}{\textbf{edge<}}\textcolor{deepred}{n\_i11}\textcolor{black}{\textbf{,}} \textcolor{deepred}{n\_ibr}\textcolor{black}{\textbf{>}} \textcolor{deepred}{e\_10\_br}\textcolor{black}{\textbf{:}} \textcolor{deepred}{E}\textcolor{deepred}{\_sw}
  \textcolor{black}{\textbf{set-switch}} \textcolor{deepred}{n\_ibr} \textcolor{black}{\textbf{when}} \textcolor{green}{sw==1}
  ...
\textcolor{black}{\textbf{\}}}
\end{Verbatim}
}

==> gen-specs/lang-cnn-relations.tex <==
{
\setlength{\tabcolsep}{1pt}
\footnotesize
\begin{tabular}{lccl}
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{FlowE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Inp}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{IdealV}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \cdot \textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{g}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{FlowE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Inp}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{IdealV}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{s}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $0.0$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{MapE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{IdealV}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Out}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{fn}}}{\left(\textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \right)}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{MapE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{IdealV}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{IdealV}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{s}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} + \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{z}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{FlowE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Out}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{IdealV}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \cdot \textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{g}}}$\\
\end{tabular}
}

==> gen-specs/lang-cnn-types.tex <==
{\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\footnotesize,fontseries=b]
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{1}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{IdealV} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{z} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}} \textcolor{black}{\textbf{\}}}
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{Out} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} \textcolor{black}{\textbf{\}}}
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{1}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{Inp} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{\}}}
\textcolor{black}{\textbf{edge-type}} \textcolor{deepred}{MapE} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{\}}}
\textcolor{black}{\textbf{edge-type}} \textcolor{deepred}{FlowE} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{g} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}} \textcolor{black}{\textbf{\}}}
\end{Verbatim}
}

==> gen-specs/lang-cnn-validation.tex <==
{
\setlength{\tabcolsep}{1pt}
\footnotesize
\begin{tabular}{lll}
\multicolumn{3}{l}{\textbf{\texttt{\textcolor{black}{\textbf{cstr}}}} \textbf{\texttt{\textcolor{deepred}{IdealV}}} \{}\\
 & \textbf{\texttt{\textcolor{black}{\textbf{acc}}}} & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{MapE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{IdealV}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}[\textbf{\texttt{\textcolor{deepred}{Out}}}]\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{4}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{9}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{FlowE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} [\textbf{\texttt{\textcolor{deepred}{Out}}}]\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{IdealV}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{FlowE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{IdealV}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
\multicolumn{3}{l}{\}}\\
\multicolumn{3}{l}{\textbf{\texttt{\textcolor{black}{\textbf{cstr}}}} \textbf{\texttt{\textcolor{deepred}{Out}}} \{}\\
 & \textbf{\texttt{\textcolor{black}{\textbf{acc}}}} & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{4}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{9}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{FlowE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Out}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}[\textbf{\texttt{\textcolor{deepred}{IdealV}}}]\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{MapE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} [\textbf{\texttt{\textcolor{deepred}{IdealV}}}]\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{Out}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
\multicolumn{3}{l}{\}}\\
\multicolumn{3}{l}{\textbf{\texttt{\textcolor{black}{\textbf{cstr}}}} \textbf{\texttt{\textcolor{deepred}{Inp}}} \{}\\
 & \textbf{\texttt{\textcolor{black}{\textbf{acc}}}} & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{4}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{9}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{FlowE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Inp}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}[\textbf{\texttt{\textcolor{deepred}{IdealV}}}]\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
\multicolumn{3}{l}{\}}\\
\end{tabular}
}

==> gen-specs/lang-con-intercon-language.tex <==
{
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\footnotesize,fontseries=b]
\textcolor{ultraviolet}{\textbf{lang}} \textcolor{deepblue}{con-intercon} \textcolor{black}{\textbf{\{}}
  \textcolor{ultraviolet}{\textbf{node-type}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{ultraviolet}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepblue}{Osc}
  \textcolor{black}{\textbf{\{}}\textcolor{ultraviolet}{\textbf{attr}} \textcolor{burntorange}{lock\_fn} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{lambd}}\textcolor{black}{\textbf{(}}\textcolor{deepblue}{a0}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
    \textcolor{ultraviolet}{\textbf{attr}} \textcolor{burntorange}{osc\_fn} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{lambd}}\textcolor{black}{\textbf{(}}\textcolor{deepblue}{a0}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{edge-type}} \textcolor{deepblue}{Cpl} \textcolor{black}{\textbf{\{}}\textcolor{ultraviolet}{\textbf{attr}} \textcolor{burntorange}{k} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Cpl}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Osc}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Osc}\textcolor{black}{\textbf{)}}
    \textcolor{burntorange}{s}\textcolor{black}{\textbf{\textless{}=}}$- \textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{k} \cdot \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{osc\_fn}{\left(\textcolor{ultraviolet}{\textbf{var(}}\textcolor{burntorange}{s}\textcolor{black}{\textbf{)}} - \textcolor{ultraviolet}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} \right)}$\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Cpl}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Osc}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Osc}\textcolor{black}{\textbf{)}}
    \textcolor{burntorange}{t}\textcolor{black}{\textbf{\textless{}=}}$- \textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{k} \cdot \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{osc\_fn}{\left(- \textcolor{ultraviolet}{\textbf{var(}}\textcolor{burntorange}{s}\textcolor{black}{\textbf{)}} + \textcolor{ultraviolet}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} \right)}$\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Cpl}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Osc}\textcolor{black}{\textbf{)}}
    \textcolor{burntorange}{s}\textcolor{black}{\textbf{\textless{}=}}$- \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{lock\_fn}{\left(\textcolor{ultraviolet}{\textbf{time}},\textcolor{ultraviolet}{\textbf{var(}}\textcolor{burntorange}{s}\textcolor{black}{\textbf{)}} \right)}$\textcolor{black}{\textbf{;}}
   \textcolor{black}{\textbf{\}}}
\end{Verbatim}
}

==> gen-specs/lang-con-intercon-relations.tex <==
{
\setlength{\tabcolsep}{1pt}
\footnotesize
\begin{tabular}{lccl}
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Coupling}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Osc}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Osc}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{s}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $- \textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{k}}} \cdot \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{osc\_fn}}}{\left(\textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} - \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \right)}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Coupling}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Osc}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Osc}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $- \textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{k}}} \cdot \textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{osc\_fn}}}{\left(- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} + \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \right)}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Coupling}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Osc}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Osc}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{s}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $- \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{lock\_fn}}}{\left(\textbf{\texttt{\textcolor{black}{\textbf{time}}}},\textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \right)}$\\
\end{tabular}
}

==> gen-specs/lang-con-intercon-types.tex <==
{\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\footnotesize,fontseries=b]
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{1}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{Osc} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{lock\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} , \textcolor{black}{\textbf{attr}} \textcolor{deepred}{osc\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} \textcolor{black}{\textbf{\}}}
\textcolor{black}{\textbf{edge-type}} \textcolor{deepred}{Coupling} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{k} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}} \textcolor{black}{\textbf{\}}}
\end{Verbatim}
}

==> gen-specs/lang-con-types.tex <==
{\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\footnotesize,fontseries=b]
\textcolor{black}{\textbf{node-type}} \textcolor{deepblue}{Osc} \textcolor{black}{\textbf{order(}}\textcolor{deepblue}{1}\textcolor{black}{\textbf{)}} \textcolor{black}{\textbf{reduce(}}\textcolor{deepblue}{+}\textcolor{black}{\textbf{)}} \textcolor{black}{\textbf{{}}
\textcolor{black}{\textbf{attr}}\textcolor{deepblue}{lock\_fn}\textcolor{black}{\textbf{:}}\textcolor{deepred}{func} , \textcolor{black}{\textbf{attr}}\textcolor{deepblue}{osc\_fn}\textcolor{black}{\textbf{:}}\textcolor{deepred}{func} \textcolor{black}{\textbf{}}}
\textcolor{black}{\textbf{edge-type}} \textcolor{deepblue}{Coupling} \textcolor{black}{\textbf{{}}
\textcolor{black}{\textbf{attr}}\textcolor{deepblue}{k}\textcolor{black}{\textbf{:}}\textcolor{deepred}{func} \textcolor{black}{\textbf{}}}
\end{Verbatim}
}

==> gen-specs/lang-hw-cnn-relations.tex <==
{
\setlength{\tabcolsep}{1pt}
\footnotesize
\begin{tabular}{lccl}
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{burntorange}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{burntorange}{fE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{burntorange}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{burntorange}{Inp}}}\textbf{\texttt{\textcolor{black}{\textbf{-\textgreater{}}}}}\textbf{\texttt{\textcolor{burntorange}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{burntorange}{Vm}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{burntorange}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{\textless{}=}}}} & $\textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{burntorange}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \cdot \textbf{\texttt{\textcolor{burntorange}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{burntorange}{g}}} \cdot \textbf{\texttt{\textcolor{burntorange}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{burntorange}{mm}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{burntorange}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{burntorange}{iE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{burntorange}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{burntorange}{Vm}}}\textbf{\texttt{\textcolor{black}{\textbf{-\textgreater{}}}}}\textbf{\texttt{\textcolor{burntorange}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{burntorange}{Vm}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{burntorange}{s}}} & \textbf{\texttt{\textcolor{black}{\textbf{\textless{}=}}}} & $\textbf{\texttt{\textcolor{burntorange}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{burntorange}{mm}}} \cdot \left(- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{burntorange}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} + \textbf{\texttt{\textcolor{burntorange}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{burntorange}{z}}}\right)$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{burntorange}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{burntorange}{fE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{burntorange}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{burntorange}{Out}}}\textbf{\texttt{\textcolor{black}{\textbf{-\textgreater{}}}}}\textbf{\texttt{\textcolor{burntorange}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{burntorange}{Vm}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{burntorange}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{\textless{}=}}}} & $\textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{burntorange}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \cdot \textbf{\texttt{\textcolor{burntorange}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{burntorange}{g}}} \cdot \textbf{\texttt{\textcolor{burntorange}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{burntorange}{mm}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{burntorange}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{burntorange}{iE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{burntorange}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{burntorange}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{-\textgreater{}}}}}\textbf{\texttt{\textcolor{burntorange}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{burntorange}{Out}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{burntorange}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{\textless{}=}}}} & $\textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{burntorange}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} + \textbf{\texttt{\textcolor{burntorange}{sat\_ni}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{burntorange}{x}}}$\\
\end{tabular}
}

==> gen-specs/lang-hwcnn-relations.tex <==
{
\setlength{\tabcolsep}{1pt}
\footnotesize
\begin{tabular}{lccl}
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{FlowE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Inp}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{MmV}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \cdot \textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{g}}} \cdot \textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{mm}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{MapE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{MmV}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{MmV}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{s}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{mm}}} \cdot \left(- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} + \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{z}}}\right)$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{FlowE}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Out}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{MmV}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \cdot \textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{g}}} \cdot \textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{mm}}}$\\
\end{tabular}
}

==> gen-specs/lang-hwcnn-types.tex <==
{\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\footnotesize,fontseries=b]
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{1}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{IdealV} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{z} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}} \textcolor{black}{\textbf{\}}}
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{Out} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} \textcolor{black}{\textbf{\}}}
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{1}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{Inp} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{\}}}
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{1}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{MmV} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{z} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}} , \textcolor{black}{\textbf{attr}} \textcolor{deepred}{mm} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}} \textcolor{black}{\textbf{\}}} \textcolor{black}{\textbf{inherit}} \textcolor{deepred}{IdealV}
\textcolor{black}{\textbf{edge-type}} \textcolor{deepred}{MapE} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{\}}}
\textcolor{black}{\textbf{edge-type}} \textcolor{deepred}{FlowE} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{g} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}} \textcolor{black}{\textbf{\}}}
\textcolor{black}{\textbf{edge-type}} \textcolor{deepred}{MmFlowE\_1p} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{g} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}} \textcolor{black}{\textbf{\}}} \textcolor{black}{\textbf{inherit}} \textcolor{deepred}{FlowE}
\textcolor{black}{\textbf{edge-type}} \textcolor{deepred}{MmFlowE\_10p} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{g} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}} \textcolor{black}{\textbf{\}}} \textcolor{black}{\textbf{inherit}} \textcolor{deepred}{FlowE}
\end{Verbatim}
}

==> gen-specs/lang-hwcon-intercon-language.tex <==
{
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\footnotesize,fontseries=b]
\textcolor{ultraviolet}{\textbf{lang}} \textcolor{deepblue}{hwcon-intercon} \textcolor{ultraviolet}{\textbf{inherits}} \textcolor{deepblue}{con-intercon}\textcolor{black}{\textbf{\{}}
  \textcolor{ultraviolet}{\textbf{node-type}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{ultraviolet}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepblue}{Osc\_G0} \textcolor{ultraviolet}{\textbf{inherit}} \textcolor{deepblue}{Osc}
  \textcolor{black}{\textbf{\{}}\textcolor{ultraviolet}{\textbf{attr}} \textcolor{burntorange}{lock\_fn} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{lambd}}\textcolor{black}{\textbf{(}}\textcolor{deepblue}{a0}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
    \textcolor{ultraviolet}{\textbf{attr}} \textcolor{burntorange}{osc\_fn} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{lambd}}\textcolor{black}{\textbf{(}}\textcolor{deepblue}{a0}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{node-type}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{ultraviolet}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepblue}{Osc\_G1} \textcolor{ultraviolet}{\textbf{inherit}} \textcolor{deepblue}{Osc}
  \textcolor{black}{\textbf{\{}}\textcolor{ultraviolet}{\textbf{attr}} \textcolor{burntorange}{lock\_fn} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{lambd}}\textcolor{black}{\textbf{(}}\textcolor{deepblue}{a0}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
    \textcolor{ultraviolet}{\textbf{attr}} \textcolor{burntorange}{osc\_fn} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{lambd}}\textcolor{black}{\textbf{(}}\textcolor{deepblue}{a0}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{node-type}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{ultraviolet}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepblue}{Osc\_G2} \textcolor{ultraviolet}{\textbf{inherit}} \textcolor{deepblue}{Osc}
  \textcolor{black}{\textbf{\{}}\textcolor{ultraviolet}{\textbf{attr}} \textcolor{burntorange}{lock\_fn} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{lambd}}\textcolor{black}{\textbf{(}}\textcolor{deepblue}{a0}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
    \textcolor{ultraviolet}{\textbf{attr}} \textcolor{burntorange}{osc\_fn} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{lambd}}\textcolor{black}{\textbf{(}}\textcolor{deepblue}{a0}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{node-type}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{ultraviolet}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepblue}{Osc\_G3} \textcolor{ultraviolet}{\textbf{inherit}} \textcolor{deepblue}{Osc}
  \textcolor{black}{\textbf{\{}}\textcolor{ultraviolet}{\textbf{attr}} \textcolor{burntorange}{lock\_fn} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{lambd}}\textcolor{black}{\textbf{(}}\textcolor{deepblue}{a0}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
    \textcolor{ultraviolet}{\textbf{attr}} \textcolor{burntorange}{osc\_fn} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{lambd}}\textcolor{black}{\textbf{(}}\textcolor{deepblue}{a0}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{edge-type}} \textcolor{deepblue}{Coupling\_l} \textcolor{ultraviolet}{\textbf{inherit}} \textcolor{deepblue}{Coupling}
  \textcolor{black}{\textbf{\{}}\textcolor{ultraviolet}{\textbf{attr}} \textcolor{burntorange}{k} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}
    \textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{edge-type}} \textcolor{deepblue}{Coupling\_g} \textcolor{ultraviolet}{\textbf{inherit}} \textcolor{deepblue}{Coupling}
  \textcolor{black}{\textbf{\{}}\textcolor{ultraviolet}{\textbf{attr}} \textcolor{burntorange}{k} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}
    \textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{cstr}} \textcolor{burntorange}{Osc\_G0} \textcolor{black}{\textbf{\{}}\textcolor{ultraviolet}{\textbf{acc}}\textcolor{black}{\textbf{[}}\textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{1}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_l}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{Osc\_G0}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{ultraviolet}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_l}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Osc\_G0}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{Osc\_G0}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{ultraviolet}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_l}\textcolor{black}{\textbf{,}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{Osc\_G0}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{burntorange}{Osc\_G0}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{ultraviolet}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_g}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Osc\_G0}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{Osc}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{ultraviolet}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_g}\textcolor{black}{\textbf{,}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{Osc}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{burntorange}{Osc\_G0}\textcolor{black}{\textbf{)}}
      \textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{\}}}
  \textcolor{ultraviolet}{\textbf{cstr}} \textcolor{burntorange}{Osc\_G1} \textcolor{black}{\textbf{\{}}\textcolor{ultraviolet}{\textbf{acc}}\textcolor{black}{\textbf{[}}\textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{1}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_l}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{Osc\_G1}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{ultraviolet}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_l}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Osc\_G1}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{Osc\_G1}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{ultraviolet}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_l}\textcolor{black}{\textbf{,}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{Osc\_G1}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{burntorange}{Osc\_G1}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{ultraviolet}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_g}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Osc\_G1}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{Osc}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{ultraviolet}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_g}\textcolor{black}{\textbf{,}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{Osc}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{burntorange}{Osc\_G1}\textcolor{black}{\textbf{)}}
      \textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{\}}}
  \textcolor{ultraviolet}{\textbf{cstr}} \textcolor{burntorange}{Osc\_G2} \textcolor{black}{\textbf{\{}}\textcolor{ultraviolet}{\textbf{acc}}\textcolor{black}{\textbf{[}}\textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{1}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_l}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{Osc\_G2}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{ultraviolet}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_l}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Osc\_G2}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{Osc\_G2}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{ultraviolet}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_l}\textcolor{black}{\textbf{,}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{Osc\_G2}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{burntorange}{Osc\_G2}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{ultraviolet}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_g}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Osc\_G2}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{Osc}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{ultraviolet}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_g}\textcolor{black}{\textbf{,}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{Osc}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{burntorange}{Osc\_G2}\textcolor{black}{\textbf{)}}
      \textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{\}}}
  \textcolor{ultraviolet}{\textbf{cstr}} \textcolor{burntorange}{Osc\_G3} \textcolor{black}{\textbf{\{}}\textcolor{ultraviolet}{\textbf{acc}}\textcolor{black}{\textbf{[}}\textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{1}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_l}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{Osc\_G3}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{ultraviolet}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_l}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Osc\_G3}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{Osc\_G3}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{ultraviolet}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_l}\textcolor{black}{\textbf{,}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{Osc\_G3}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{burntorange}{Osc\_G3}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{ultraviolet}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_g}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Osc\_G3}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{Osc}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{ultraviolet}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{Coupling\_g}\textcolor{black}{\textbf{,}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{Osc}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{burntorange}{Osc\_G3}\textcolor{black}{\textbf{)}}
      \textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{\}}}
   \textcolor{black}{\textbf{\}}}
\end{Verbatim}
}

==> gen-specs/lang-hwcon-intercon-types.tex <==
{\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\footnotesize,fontseries=b]
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{1}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{Osc} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{lock\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} , \textcolor{black}{\textbf{attr}} \textcolor{deepred}{osc\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} \textcolor{black}{\textbf{\}}}
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{1}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{Osc\_G0} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{lock\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} , \textcolor{black}{\textbf{attr}} \textcolor{deepred}{osc\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} \textcolor{black}{\textbf{\}}} \textcolor{black}{\textbf{inherit}} \textcolor{deepred}{Osc}
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{1}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{Osc\_G1} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{lock\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} , \textcolor{black}{\textbf{attr}} \textcolor{deepred}{osc\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} \textcolor{black}{\textbf{\}}} \textcolor{black}{\textbf{inherit}} \textcolor{deepred}{Osc}
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{1}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{Osc\_G2} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{lock\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} , \textcolor{black}{\textbf{attr}} \textcolor{deepred}{osc\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} \textcolor{black}{\textbf{\}}} \textcolor{black}{\textbf{inherit}} \textcolor{deepred}{Osc}
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{1}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{Osc\_G3} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{lock\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} , \textcolor{black}{\textbf{attr}} \textcolor{deepred}{osc\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} \textcolor{black}{\textbf{\}}} \textcolor{black}{\textbf{inherit}} \textcolor{deepred}{Osc}
\textcolor{black}{\textbf{edge-type}} \textcolor{deepred}{Coupling} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{k} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}} \textcolor{black}{\textbf{\}}}
\textcolor{black}{\textbf{edge-type}} \textcolor{deepred}{Coupling\_l} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{k} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}} \textcolor{black}{\textbf{\}}} \textcolor{black}{\textbf{inherit}} \textcolor{deepred}{Coupling}
\textcolor{black}{\textbf{edge-type}} \textcolor{deepred}{Coupling\_g} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{k} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}} \textcolor{black}{\textbf{\}}} \textcolor{black}{\textbf{inherit}} \textcolor{deepred}{Coupling}
\end{Verbatim}
}

==> gen-specs/lang-hwcon-intercon-validation.tex <==
{
\setlength{\tabcolsep}{1pt}
\footnotesize
\begin{tabular}{lll}
\multicolumn{3}{l}{\textbf{\texttt{\textcolor{black}{\textbf{cstr}}}} \textbf{\texttt{\textcolor{deepred}{Osc\_G0}}} \{}\\
 & \textbf{\texttt{\textcolor{black}{\textbf{acc}}}} & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_l}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Osc\_G0}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_l}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Osc\_G0}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}[\textbf{\texttt{\textcolor{deepred}{Osc\_G0}}}]\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_l}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} [\textbf{\texttt{\textcolor{deepred}{Osc\_G0}}}]\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{Osc\_G0}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_g}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Osc\_G0}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}[\textbf{\texttt{\textcolor{deepred}{Osc}}}]\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_g}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} [\textbf{\texttt{\textcolor{deepred}{Osc}}}]\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{Osc\_G0}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
\multicolumn{3}{l}{\}}\\
\multicolumn{3}{l}{\textbf{\texttt{\textcolor{black}{\textbf{cstr}}}} \textbf{\texttt{\textcolor{deepred}{Osc\_G1}}} \{}\\
 & \textbf{\texttt{\textcolor{black}{\textbf{acc}}}} & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_l}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Osc\_G1}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_l}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Osc\_G1}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}[\textbf{\texttt{\textcolor{deepred}{Osc\_G1}}}]\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_l}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} [\textbf{\texttt{\textcolor{deepred}{Osc\_G1}}}]\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{Osc\_G1}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_g}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Osc\_G1}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}[\textbf{\texttt{\textcolor{deepred}{Osc}}}]\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_g}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} [\textbf{\texttt{\textcolor{deepred}{Osc}}}]\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{Osc\_G1}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
\multicolumn{3}{l}{\}}\\
\multicolumn{3}{l}{\textbf{\texttt{\textcolor{black}{\textbf{cstr}}}} \textbf{\texttt{\textcolor{deepred}{Osc\_G2}}} \{}\\
 & \textbf{\texttt{\textcolor{black}{\textbf{acc}}}} & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_l}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Osc\_G2}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_l}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Osc\_G2}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}[\textbf{\texttt{\textcolor{deepred}{Osc\_G2}}}]\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_l}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} [\textbf{\texttt{\textcolor{deepred}{Osc\_G2}}}]\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{Osc\_G2}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_g}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Osc\_G2}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}[\textbf{\texttt{\textcolor{deepred}{Osc}}}]\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_g}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} [\textbf{\texttt{\textcolor{deepred}{Osc}}}]\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{Osc\_G2}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
\multicolumn{3}{l}{\}}\\
\multicolumn{3}{l}{\textbf{\texttt{\textcolor{black}{\textbf{cstr}}}} \textbf{\texttt{\textcolor{deepred}{Osc\_G3}}} \{}\\
 & \textbf{\texttt{\textcolor{black}{\textbf{acc}}}} & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_l}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Osc\_G3}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_l}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Osc\_G3}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}[\textbf{\texttt{\textcolor{deepred}{Osc\_G3}}}]\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_l}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} [\textbf{\texttt{\textcolor{deepred}{Osc\_G3}}}]\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{Osc\_G3}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_g}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Osc\_G3}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}[\textbf{\texttt{\textcolor{deepred}{Osc}}}]\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{Coupling\_g}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} [\textbf{\texttt{\textcolor{deepred}{Osc}}}]\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{Osc\_G3}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
\multicolumn{3}{l}{\}}\\
\end{tabular}
}

==> gen-specs/lang-hwtln-language.tex <==
{
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\footnotesize,fontseries=b]
\textcolor{ultraviolet}{\textbf{lang}} \textcolor{deepblue}{hwtln} \textcolor{ultraviolet}{\textbf{inherits}} \textcolor{deepblue}{tln}\textcolor{black}{\textbf{\{}}
  \textcolor{ultraviolet}{\textbf{node-type}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepblue}{Vm}\textcolor{black}{\textbf{inherit}}\textcolor{deepblue}{V}
  \textcolor{black}{\textbf{\{}}\textcolor{black}{\textbf{attr}} \textcolor{burntorange}{c} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{1e-10}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1e-08}\textcolor{black}{\textbf{]}} \textcolor{black}{\textbf{mismatch(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{0.1}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
    \textcolor{black}{\textbf{attr}} \textcolor{burntorange}{g} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{inf}}\textcolor{black}{\textbf{]}}
    \textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{node-type}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepblue}{Im}\textcolor{black}{\textbf{inherit}}\textcolor{deepblue}{I}
  \textcolor{black}{\textbf{\{}}\textcolor{black}{\textbf{attr}} \textcolor{burntorange}{l} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{1e-10}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1e-08}\textcolor{black}{\textbf{]}} \textcolor{black}{\textbf{mismatch(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{0.1}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
    \textcolor{black}{\textbf{attr}} \textcolor{burntorange}{r} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{inf}}\textcolor{black}{\textbf{]}}
    \textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{edge-type}} \textcolor{deepblue}{Em}\textcolor{black}{\textbf{inherit}}\textcolor{deepblue}{E}
  \textcolor{black}{\textbf{\{}}\textcolor{black}{\textbf{attr}} \textcolor{burntorange}{ws} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{0.5}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{2}\textcolor{black}{\textbf{]}} \textcolor{black}{\textbf{mismatch(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{0.1}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
    \textcolor{black}{\textbf{attr}} \textcolor{burntorange}{wt} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{0.5}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{2}\textcolor{black}{\textbf{]}} \textcolor{black}{\textbf{mismatch(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{0.1}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Em}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{)}} \textcolor{black}{\textbf{s}}\textcolor{black}{\textbf{\textless{}=}}$- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} \cdot \textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{ws} / \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{c}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Em}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\textcolor{black}{\textbf{var(}}\textcolor{burntorange}{s}\textcolor{black}{\textbf{)}} \cdot \textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{wt} / \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{l}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Em}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{s}}\textcolor{black}{\textbf{\textless{}=}}$- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} \cdot \textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{ws} / \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{l}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Em}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\textcolor{black}{\textbf{var(}}\textcolor{burntorange}{s}\textcolor{black}{\textbf{)}} \cdot \textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{wt} / \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{c}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Em}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{InpV}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\frac{\textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{wt} \cdot \left(- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} + \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{fn}{\left(\textcolor{black}{\textbf{time}} \right)}\right)}{\textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{r} \cdot \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{c}}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Em}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{InpV}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{wt} \cdot \left(- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} \cdot \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{r} + \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{fn}{\left(\textcolor{black}{\textbf{time}} \right)}\right) / \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{l}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Em}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{InpI}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{wt} \cdot \left(- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} \cdot \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{g} + \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{fn}{\left(\textcolor{black}{\textbf{time}} \right)}\right) / \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{c}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Em}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{InpI}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\frac{\textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{wt} \cdot \left(- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} + \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{fn}{\left(\textcolor{black}{\textbf{time}} \right)}\right)}{\textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{g} \cdot \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{l}}$\textcolor{black}{\textbf{;}}
  
\textcolor{black}{\textbf{\}}}
\end{Verbatim}
}

==> gen-specs/lang-hwtln-relations.tex <==
{
\setlength{\tabcolsep}{1pt}
\footnotesize
\begin{tabular}{lccl}
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Em}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{I}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{s}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \cdot \textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{ws}}} / \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{c}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Em}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{I}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \cdot \textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{wt}}} / \textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{l}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Em}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{I}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{s}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \cdot \textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{ws}}} / \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{l}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Em}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{I}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \cdot \textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{wt}}} / \textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{c}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Em}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{InpV}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\frac{\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{wt}}} \cdot \left(- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} + \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{fn}}}{\left(\textbf{\texttt{\textcolor{black}{\textbf{time}}}} \right)}\right)}{\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{r}}} \cdot \textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{c}}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Em}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{InpV}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{I}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{wt}}} \cdot \left(- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \cdot \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{r}}} + \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{fn}}}{\left(\textbf{\texttt{\textcolor{black}{\textbf{time}}}} \right)}\right) / \textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{l}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Em}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{InpI}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{wt}}} \cdot \left(- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \cdot \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{g}}} + \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{fn}}}{\left(\textbf{\texttt{\textcolor{black}{\textbf{time}}}} \right)}\right) / \textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{c}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Em}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{InpI}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{I}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\frac{\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{wt}}} \cdot \left(- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} + \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{fn}}}{\left(\textbf{\texttt{\textcolor{black}{\textbf{time}}}} \right)}\right)}{\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{g}}} \cdot \textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{l}}}}$\\
\end{tabular}
}

==> gen-specs/lang-hwtln-types.tex <==
{\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\footnotesize,fontseries=b]
\textbf{\texttt{\textcolor{black}{\textbf{node-type(}}}}\textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{sum}}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \textbf{\texttt{\textcolor{deepred}{V}}} \textbf{\texttt{\textcolor{black}{\textbf{\{}}}} \textbf{\texttt{\textcolor{black}{\textbf{attr}}}} \textbf{\texttt{\textcolor{deepred}{c}}} \textbf{\texttt{\textcolor{black}{\textbf{=}}}} \textbf{\texttt{\textcolor{black}{\textbf{real}}}}\textbf{\texttt{\textcolor{black}{\textbf{[}}}}\textbf{\texttt{\textcolor{deepred}{1e-10}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1e-08}}}\textbf{\texttt{\textcolor{black}{\textbf{]}}}} , \textbf{\texttt{\textcolor{black}{\textbf{attr}}}} \textbf{\texttt{\textcolor{deepred}{g}}} \textbf{\texttt{\textcolor{black}{\textbf{=}}}} \textbf{\texttt{\textcolor{black}{\textbf{real}}}}\textbf{\texttt{\textcolor{black}{\textbf{[}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{]}}}} \textbf{\texttt{\textcolor{black}{\textbf{\}}}}}
\textbf{\texttt{\textcolor{black}{\textbf{node-type(}}}}\textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{sum}}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \textbf{\texttt{\textcolor{deepred}{I}}} \textbf{\texttt{\textcolor{black}{\textbf{\{}}}} \textbf{\texttt{\textcolor{black}{\textbf{attr}}}} \textbf{\texttt{\textcolor{deepred}{l}}} \textbf{\texttt{\textcolor{black}{\textbf{=}}}} \textbf{\texttt{\textcolor{black}{\textbf{real}}}}\textbf{\texttt{\textcolor{black}{\textbf{[}}}}\textbf{\texttt{\textcolor{deepred}{1e-10}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1e-08}}}\textbf{\texttt{\textcolor{black}{\textbf{]}}}} , \textbf{\texttt{\textcolor{black}{\textbf{attr}}}} \textbf{\texttt{\textcolor{deepred}{r}}} \textbf{\texttt{\textcolor{black}{\textbf{=}}}} \textbf{\texttt{\textcolor{black}{\textbf{real}}}}\textbf{\texttt{\textcolor{black}{\textbf{[}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{]}}}} \textbf{\texttt{\textcolor{black}{\textbf{\}}}}}
\textbf{\texttt{\textcolor{black}{\textbf{node-type(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{sum}}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \textbf{\texttt{\textcolor{deepred}{InpV}}} \textbf{\texttt{\textcolor{black}{\textbf{\{}}}} \textbf{\texttt{\textcolor{black}{\textbf{attr}}}} \textbf{\texttt{\textcolor{deepred}{fn}}} \textbf{\texttt{\textcolor{black}{\textbf{=}}}} \textbf{\texttt{\textcolor{black}{\textbf{lambd}}}} , \textbf{\texttt{\textcolor{black}{\textbf{attr}}}} \textbf{\texttt{\textcolor{deepred}{r}}} \textbf{\texttt{\textcolor{black}{\textbf{=}}}} \textbf{\texttt{\textcolor{black}{\textbf{real}}}}\textbf{\texttt{\textcolor{black}{\textbf{[}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{]}}}} \textbf{\texttt{\textcolor{black}{\textbf{\}}}}}
\textbf{\texttt{\textcolor{black}{\textbf{node-type(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{sum}}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \textbf{\texttt{\textcolor{deepred}{InpI}}} \textbf{\texttt{\textcolor{black}{\textbf{\{}}}} \textbf{\texttt{\textcolor{black}{\textbf{attr}}}} \textbf{\texttt{\textcolor{deepred}{fn}}} \textbf{\texttt{\textcolor{black}{\textbf{=}}}} \textbf{\texttt{\textcolor{black}{\textbf{lambd}}}} , \textbf{\texttt{\textcolor{black}{\textbf{attr}}}} \textbf{\texttt{\textcolor{deepred}{g}}} \textbf{\texttt{\textcolor{black}{\textbf{=}}}} \textbf{\texttt{\textcolor{black}{\textbf{real}}}}\textbf{\texttt{\textcolor{black}{\textbf{[}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{]}}}} \textbf{\texttt{\textcolor{black}{\textbf{\}}}}}
\textbf{\texttt{\textcolor{black}{\textbf{node-type(}}}}\textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{sum}}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \textbf{\texttt{\textcolor{deepred}{Vm}}} \textbf{\texttt{\textcolor{black}{\textbf{\{}}}} \textbf{\texttt{\textcolor{black}{\textbf{attr}}}} \textbf{\texttt{\textcolor{deepred}{c}}} \textbf{\texttt{\textcolor{black}{\textbf{=}}}} \textbf{\texttt{\textcolor{black}{\textbf{real}}}}\textbf{\texttt{\textcolor{black}{\textbf{[}}}}\textbf{\texttt{\textcolor{deepred}{1e-10}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1e-08}}}\textbf{\texttt{\textcolor{black}{\textbf{]}}}} \textbf{\texttt{\textcolor{black}{\textbf{mismatch(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{0.1}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} , \textbf{\texttt{\textcolor{black}{\textbf{attr}}}} \textbf{\texttt{\textcolor{deepred}{g}}} \textbf{\texttt{\textcolor{black}{\textbf{=}}}} \textbf{\texttt{\textcolor{black}{\textbf{real}}}}\textbf{\texttt{\textcolor{black}{\textbf{[}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{]}}}} \textbf{\texttt{\textcolor{black}{\textbf{\}}}}} \textbf{\texttt{\textcolor{black}{\textbf{inherit}}}} \textbf{\texttt{\textcolor{deepred}{V}}}
\textbf{\texttt{\textcolor{black}{\textbf{node-type(}}}}\textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{sum}}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \textbf{\texttt{\textcolor{deepred}{Im}}} \textbf{\texttt{\textcolor{black}{\textbf{\{}}}} \textbf{\texttt{\textcolor{black}{\textbf{attr}}}} \textbf{\texttt{\textcolor{deepred}{l}}} \textbf{\texttt{\textcolor{black}{\textbf{=}}}} \textbf{\texttt{\textcolor{black}{\textbf{real}}}}\textbf{\texttt{\textcolor{black}{\textbf{[}}}}\textbf{\texttt{\textcolor{deepred}{1e-10}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1e-08}}}\textbf{\texttt{\textcolor{black}{\textbf{]}}}} \textbf{\texttt{\textcolor{black}{\textbf{mismatch(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{0.1}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} , \textbf{\texttt{\textcolor{black}{\textbf{attr}}}} \textbf{\texttt{\textcolor{deepred}{r}}} \textbf{\texttt{\textcolor{black}{\textbf{=}}}} \textbf{\texttt{\textcolor{black}{\textbf{real}}}}\textbf{\texttt{\textcolor{black}{\textbf{[}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{]}}}} \textbf{\texttt{\textcolor{black}{\textbf{\}}}}} \textbf{\texttt{\textcolor{black}{\textbf{inherit}}}} \textbf{\texttt{\textcolor{deepred}{I}}}
\textbf{\texttt{\textcolor{black}{\textbf{edge-type}}}} \textbf{\texttt{\textcolor{deepred}{E}}} \textbf{\texttt{\textcolor{black}{\textbf{\{}}}} \textbf{\texttt{\textcolor{black}{\textbf{\}}}}}
\textbf{\texttt{\textcolor{black}{\textbf{edge-type}}}} \textbf{\texttt{\textcolor{deepred}{Em}}} \textbf{\texttt{\textcolor{black}{\textbf{\{}}}} \textbf{\texttt{\textcolor{black}{\textbf{attr}}}} \textbf{\texttt{\textcolor{deepred}{ws}}} \textbf{\texttt{\textcolor{black}{\textbf{=}}}} \textbf{\texttt{\textcolor{black}{\textbf{real}}}}\textbf{\texttt{\textcolor{black}{\textbf{[}}}}\textbf{\texttt{\textcolor{deepred}{0.5}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{2}}}\textbf{\texttt{\textcolor{black}{\textbf{]}}}} \textbf{\texttt{\textcolor{black}{\textbf{mismatch(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{0.1}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} , \textbf{\texttt{\textcolor{black}{\textbf{attr}}}} \textbf{\texttt{\textcolor{deepred}{wt}}} \textbf{\texttt{\textcolor{black}{\textbf{=}}}} \textbf{\texttt{\textcolor{black}{\textbf{real}}}}\textbf{\texttt{\textcolor{black}{\textbf{[}}}}\textbf{\texttt{\textcolor{deepred}{0.5}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{2}}}\textbf{\texttt{\textcolor{black}{\textbf{]}}}} \textbf{\texttt{\textcolor{black}{\textbf{mismatch(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{0.1}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \textbf{\texttt{\textcolor{black}{\textbf{\}}}}} \textbf{\texttt{\textcolor{black}{\textbf{inherit}}}} \textbf{\texttt{\textcolor{deepred}{E}}}
\end{Verbatim}
}

==> gen-specs/lang-obc-relations.tex <==
{
\setlength{\tabcolsep}{1pt}
\footnotesize
\begin{tabular}{lccl}
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Coupling}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Osc}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Osc}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{s}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $- \textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{k}}} \cdot \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{osc\_fn}}}{\left(\textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} - \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \right)}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Coupling}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Osc}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Osc}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $- \textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{k}}} \cdot \textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{osc\_fn}}}{\left(- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} + \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \right)}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Coupling}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Osc1}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Osc1}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{s}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $- \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{lock\_fn}}}{\left(\textbf{\texttt{\textcolor{black}{\textbf{time}}}},\textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}},100000.000000000,0.000100000000000000 \right)} - \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{noise\_fn}}}{\left(100.000000000000 \right)}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Coupling}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Osc2}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{Osc2}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{s}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $- \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{lock\_fn}}}{\left(\textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \right)} - \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{noise\_fn}}}{\left(100.000000000000 \right)}$\\
\end{tabular}
}

==> gen-specs/lang-obc-types.tex <==
{\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\footnotesize,fontseries=b]
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{1}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{Osc} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{lock\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} , \textcolor{black}{\textbf{attr}} \textcolor{deepred}{osc\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} , \textcolor{black}{\textbf{attr}} \textcolor{deepred}{noise\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} \textcolor{black}{\textbf{\}}}
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{1}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{Osc1} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{lock\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} , \textcolor{black}{\textbf{attr}} \textcolor{deepred}{osc\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} , \textcolor{black}{\textbf{attr}} \textcolor{deepred}{noise\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} \textcolor{black}{\textbf{\}}} \textcolor{black}{\textbf{inherit}} \textcolor{deepred}{Osc}
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{1}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{Osc2} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{lock\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} , \textcolor{black}{\textbf{attr}} \textcolor{deepred}{osc\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} , \textcolor{black}{\textbf{attr}} \textcolor{deepred}{noise\_fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} \textcolor{black}{\textbf{\}}} \textcolor{black}{\textbf{inherit}} \textcolor{deepred}{Osc}
\textcolor{black}{\textbf{edge-type}} \textcolor{deepred}{Coupling} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{k} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}} \textcolor{black}{\textbf{\}}}
\end{Verbatim}
}

==> gen-specs/lang-tln-relations.tex <==
{
\setlength{\tabcolsep}{1pt}
\footnotesize
\begin{tabular}{lccl}
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{I}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{s}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} / \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{c}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{I}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} / \textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{l}}}$\\
\hspace{2em}\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{I}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{s}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} / \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{l}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{I}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} / \textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{c}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{s}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \cdot \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{g}}} / \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{c}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{I}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{I}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{s}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \cdot \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{r}}} / \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{l}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{InpV}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\frac{- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} + \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{fn}}}{\left(\textbf{\texttt{\textcolor{black}{\textbf{time}}}} \right)}}{\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{r}}} \cdot \textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{c}}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{InpV}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{I}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\left(- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \cdot \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{r}}} + \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{fn}}}{\left(\textbf{\texttt{\textcolor{black}{\textbf{time}}}} \right)}\right) / \textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{l}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{InpI}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\left(- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} \cdot \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{g}}} + \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{fn}}}{\left(\textbf{\texttt{\textcolor{black}{\textbf{time}}}} \right)}\right) / \textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{c}}}$\\
\textbf{\texttt{\textcolor{black}{\textbf{prod(}}}}\textbf{\texttt{\textcolor{deepred}{e}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{InpI}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{:}}}} \textbf{\texttt{\textcolor{deepred}{I}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} & \textbf{\texttt{\textcolor{deepred}{t}}} & \textbf{\texttt{\textcolor{black}{\textbf{<=}}}} & $\frac{- \textbf{\texttt{\textcolor{black}{\textbf{var(}}}}\textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}} + \textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{fn}}}{\left(\textbf{\texttt{\textcolor{black}{\textbf{time}}}} \right)}}{\textbf{\texttt{\textcolor{deepred}{s}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{g}}} \cdot \textbf{\texttt{\textcolor{deepred}{t}}}\textbf{\texttt{\textcolor{black}{\textbf{.}}}}\textbf{\texttt{\textcolor{deepred}{l}}}}$\\
\end{tabular}
}

==> gen-specs/lang-tln-types.tex <==
    {\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\footnotesize,fontseries=b]
\textcolor{black}{\textbf{lang}} \textcolor{deepred}{tln} \{

\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{1}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{V} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{c} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{deepred}{1e-10}\textcolor{black}{\textbf{,}} \textcolor{deepred}{1e-08}\textcolor{black}{\textbf{]}} , 
                      \textcolor{black}{\textbf{attr}} \textcolor{deepred}{g} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{deepred}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{inf}}\textcolor{black}{\textbf{]}} \textcolor{black}{\textbf{\}}}
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{1}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{I} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{l} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{deepred}{1e-10}\textcolor{black}{\textbf{,}} \textcolor{deepred}{1e-08}\textcolor{black}{\textbf{]}} , 
                       \textcolor{black}{\textbf{attr}} \textcolor{deepred}{r} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{deepred}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{inf}}\textcolor{black}{\textbf{]}} \textcolor{black}{\textbf{\}}}
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{InpV} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} , 
                    \textcolor{black}{\textbf{attr}} \textcolor{deepred}{r} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{deepred}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{inf}}\textcolor{black}{\textbf{]}} \textcolor{black}{\textbf{\}}}
\textcolor{black}{\textbf{node-type(}}\textcolor{deepred}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepred}{InpI} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{attr}} \textcolor{deepred}{fn} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{lambd}} , 
                   \textcolor{black}{\textbf{attr}} \textcolor{deepred}{g} \textcolor{black}{\textbf{=}} \textcolor{black}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{deepred}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{inf}}\textcolor{black}{\textbf{]}} \textcolor{black}{\textbf{\}}}
\textcolor{black}{\textbf{edge-type}} \textcolor{deepred}{E} \textcolor{black}{\textbf{\{}} \textcolor{black}{\textbf{\}}}
\end{Verbatim}
}

==> gen-specs/lang-tln-validation.tex <==
{
\setlength{\tabcolsep}{1pt}
\footnotesize
\begin{tabular}{lll}
\multicolumn{3}{l}{
\hspace{2em}\textbf{\texttt{\textcolor{black}{\textbf{cstr}}}} \textbf{\texttt{\textcolor{deepred}{V}}} \{}\\
 & \textbf{\texttt{\textcolor{black}{\textbf{acc}}}} & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}[\textbf{\texttt{\textcolor{deepred}{I}}}]\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} [\textbf{\texttt{\textcolor{deepred}{I}}}]\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} [\textbf{\texttt{\textcolor{deepred}{InpV}}}]\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{black}{\textbf{inf}}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} [\textbf{\texttt{\textcolor{deepred}{InpI}}}]\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
\multicolumn{3}{l}{\}}\\
\multicolumn{3}{l}{\textbf{\texttt{\textcolor{black}{\textbf{cstr}}}} \textbf{\texttt{\textcolor{deepred}{I}}} \{}\\
 & \textbf{\texttt{\textcolor{black}{\textbf{acc}}}} & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{I}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}[\textbf{\texttt{\textcolor{deepred}{V}}}]\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} [\textbf{\texttt{\textcolor{deepred}{V}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{InpV}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{InpI}}}]\textbf{\texttt{\textcolor{black}{\textbf{->}}}}\textbf{\texttt{\textcolor{deepred}{I}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{I}}}\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
\multicolumn{3}{l}{\}}\\
\multicolumn{3}{l}{\textbf{\texttt{\textcolor{black}{\textbf{cstr}}}} \textbf{\texttt{\textcolor{deepred}{InpV}}} \{}\\
 & \textbf{\texttt{\textcolor{black}{\textbf{acc}}}} & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{InpV}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}[\textbf{\texttt{\textcolor{deepred}{V}}}]\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{InpV}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}[\textbf{\texttt{\textcolor{deepred}{I}}}]\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
\multicolumn{3}{l}{\}}\\
\multicolumn{3}{l}{\textbf{\texttt{\textcolor{black}{\textbf{cstr}}}} \textbf{\texttt{\textcolor{deepred}{InpI}}} \{}\\
 & \textbf{\texttt{\textcolor{black}{\textbf{acc}}}} & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{InpI}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}[\textbf{\texttt{\textcolor{deepred}{V}}}]\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
 &  & \textbf{\texttt{\textcolor{black}{\textbf{match(}}}}\textbf{\texttt{\textcolor{deepred}{0}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{1}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{E}}}\textbf{\texttt{\textcolor{black}{\textbf{,}}}} \textbf{\texttt{\textcolor{deepred}{InpI}}}\textbf{\texttt{\textcolor{black}{\textbf{->}}}}[\textbf{\texttt{\textcolor{deepred}{I}}}]\textbf{\texttt{\textcolor{black}{\textbf{)}}}}\\
\multicolumn{3}{l}{\}}\\
\multicolumn{3}{l}{\}}\\
\end{tabular}
}

==> old/tln-example/lang-hwtln-language.tex <==
{
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\footnotesize,fontseries=b]
\textcolor{ultraviolet}{\textbf{lang}} \textcolor{deepblue}{hwtln} \textcolor{ultraviolet}{\textbf{inherits}} \textcolor{deepblue}{tln}\textcolor{black}{\textbf{\{}}
  \textcolor{ultraviolet}{\textbf{node-type}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepblue}{Vm}\textcolor{black}{\textbf{inherit}}\textcolor{deepblue}{V}
  \textcolor{black}{\textbf{\{}}\textcolor{black}{\textbf{attr}} \textcolor{burntorange}{c} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{1e-10}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1e-08}\textcolor{black}{\textbf{]}} \textcolor{black}{\textbf{mismatch(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{0.1}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
    \textcolor{black}{\textbf{attr}} \textcolor{burntorange}{g} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{inf}}\textcolor{black}{\textbf{]}}
    \textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{node-type}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepblue}{Im}\textcolor{black}{\textbf{inherit}}\textcolor{deepblue}{I}
  \textcolor{black}{\textbf{\{}}\textcolor{black}{\textbf{attr}} \textcolor{burntorange}{l} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{1e-10}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1e-08}\textcolor{black}{\textbf{]}} \textcolor{black}{\textbf{mismatch(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{0.1}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
    \textcolor{black}{\textbf{attr}} \textcolor{burntorange}{r} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{inf}}\textcolor{black}{\textbf{]}}
    \textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{edge-type}} \textcolor{deepblue}{Em}\textcolor{black}{\textbf{inherit}}\textcolor{deepblue}{E}
  \textcolor{black}{\textbf{\{}}\textcolor{black}{\textbf{attr}} \textcolor{burntorange}{ws} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{0.5}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{2}\textcolor{black}{\textbf{]}} \textcolor{black}{\textbf{mismatch(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{0.1}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
    \textcolor{black}{\textbf{attr}} \textcolor{burntorange}{wt} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{0.5}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{2}\textcolor{black}{\textbf{]}} \textcolor{black}{\textbf{mismatch(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{0.1}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Em}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{s}}\textcolor{black}{\textbf{\textless{}=}}$- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} \cdot \textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{ws} / \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{c}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Em}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\textcolor{black}{\textbf{var(}}\textcolor{burntorange}{s}\textcolor{black}{\textbf{)}} \cdot \textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{wt} / \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{l}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Em}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{s}}\textcolor{black}{\textbf{\textless{}=}}$- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} \cdot \textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{ws} / \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{l}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Em}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\textcolor{black}{\textbf{var(}}\textcolor{burntorange}{s}\textcolor{black}{\textbf{)}} \cdot \textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{wt} / \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{c}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Em}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{InpV}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\frac{\textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{wt} \cdot \left(- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} + \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{fn}{\left(\textcolor{black}{\textbf{time}} \right)}\right)}{\textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{r} \cdot \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{c}}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Em}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{InpV}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{wt} \cdot \left(- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} \cdot \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{r} + \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{fn}{\left(\textcolor{black}{\textbf{time}} \right)}\right) / \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{l}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Em}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{InpI}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{wt} \cdot \left(- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} \cdot \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{g} + \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{fn}{\left(\textcolor{black}{\textbf{time}} \right)}\right) / \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{c}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{Em}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{InpI}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\frac{\textcolor{burntorange}{e}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{wt} \cdot \left(- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} + \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{fn}{\left(\textcolor{black}{\textbf{time}} \right)}\right)}{\textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{g} \cdot \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{l}}$\textcolor{black}{\textbf{;}}
  
\textcolor{black}{\textbf{\}}}
\end{Verbatim}
}

==> old/tln-example/lang-tln-br-func.tex <==
{
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\footnotesize,fontseries=b]
\textcolor{ultraviolet}{\textbf{func}} \textcolor{deepblue}{br-func} \textcolor{black}{\textbf{(}} \textcolor{deepblue}{br}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{int}\textcolor{black}{\textbf{[0,1]}}\textcolor{black}{\textbf{)}} \textcolor{ultraviolet}{\textbf{uses}} \textcolor{deepblue}{tln}\textcolor{black}{\textbf{\{}}
  \textcolor{ultraviolet}{\textbf{node}} \textcolor{deepblue}{IN\_V}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{node}} \textcolor{deepblue}{I\_0}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{node}} \textcolor{deepblue}{I\_1}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{;}} 
  \textcolor{black}{\textbf{...}}
  
  \textcolor{ultraviolet}{\textbf{edge}} \textcolor{black}{\textbf{\textless{}}}\textcolor{deepblue}{IN\_V}\textcolor{black}{\textbf{,}} \textcolor{deepblue}{I\_0}\textcolor{black}{\textbf{\textgreater{}}}\textcolor{deepblue}{E\_0}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{E}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{edge}} \textcolor{black}{\textbf{\textless{}}}\textcolor{deepblue}{I\_0}\textcolor{black}{\textbf{,}} \textcolor{deepblue}{V\_1}\textcolor{black}{\textbf{\textgreater{}}}\textcolor{deepblue}{E\_1}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{E}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{edge}} \textcolor{black}{\textbf{\textless{}}}\textcolor{deepblue}{V\_3}\textcolor{black}{\textbf{,}} \textcolor{deepblue}{V\_3}\textcolor{black}{\textbf{\textgreater{}}}\textcolor{deepblue}{E\_10}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{E}\textcolor{black}{\textbf{;}}
  
  \textcolor{black}{\textbf{...}}
  \textcolor{ultraviolet}{\textbf{set-switch}} \textcolor{deepblue}{E\_6} \textcolor{ultraviolet}{\textbf{when}} \textcolor{green}{br}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{set-attr}} \textcolor{deepblue}{IN\_V}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{c}\textcolor{black}{\textbf{=}}1e-09\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{set-attr}} \textcolor{deepblue}{IN\_V}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{g}\textcolor{black}{\textbf{=}}0.0\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{set-attr}} \textcolor{deepblue}{I\_0}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{l}\textcolor{black}{\textbf{=}}1e-09\textcolor{black}{\textbf{;}}
  
  \textcolor{black}{\textbf{...}}
  
   \textcolor{black}{\textbf{\}}}
\end{Verbatim}
}

==> old/tln-example/lang-tln-language.tex <==
{
\begin{Verbatim}[commandchars=\\\{\},codes={\catcode`$=3\catcode`_=8},fontsize=\footnotesize,fontseries=b]
\textcolor{ultraviolet}{\textbf{lang}} \textcolor{deepblue}{tln} \textcolor{black}{\textbf{\{}}
  \textcolor{ultraviolet}{\textbf{node-type}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepblue}{V}
  \textcolor{black}{\textbf{\{}}\textcolor{black}{\textbf{attr}} \textcolor{burntorange}{c} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{1e-10}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1e-08}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{,}}
    \textcolor{black}{\textbf{attr}} \textcolor{burntorange}{g} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{inf}}\textcolor{black}{\textbf{]}}
    \textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{node-type}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepblue}{I}
  \textcolor{black}{\textbf{\{}}\textcolor{black}{\textbf{attr}} \textcolor{burntorange}{l} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{1e-10}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1e-08}\textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{,}}
    \textcolor{black}{\textbf{attr}} \textcolor{burntorange}{r} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{inf}}\textcolor{black}{\textbf{]}}
    \textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{node-type}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}}\textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepblue}{InpV}
  \textcolor{black}{\textbf{\{}}\textcolor{black}{\textbf{attr}} \textcolor{burntorange}{fn} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{lambd}}\textcolor{black}{\textbf{(}}\textcolor{deepblue}{a0}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
    \textcolor{black}{\textbf{attr}} \textcolor{burntorange}{r} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{inf}}\textcolor{black}{\textbf{]}}
    \textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{ultraviolet}{\textbf{node-type}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}}\textcolor{black}{\textbf{sum}}\textcolor{black}{\textbf{)}} \textcolor{deepblue}{InpI}
  \textcolor{black}{\textbf{\{}}\textcolor{black}{\textbf{attr}} \textcolor{burntorange}{fn} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{lambd}}\textcolor{black}{\textbf{(}}\textcolor{deepblue}{a0}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
    \textcolor{black}{\textbf{attr}} \textcolor{burntorange}{g} \textcolor{black}{\textbf{=}} \textcolor{ultraviolet}{\textbf{real}}\textcolor{black}{\textbf{[}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{inf}}\textcolor{black}{\textbf{]}}
    \textcolor{black}{\textbf{\}}}\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{edge-type}} \textcolor{deepblue}{E} {}\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{E}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{s}}\textcolor{black}{\textbf{\textless{}=}}$- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} / \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{c}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{E}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\textcolor{black}{\textbf{var(}}\textcolor{burntorange}{s}\textcolor{black}{\textbf{)}} / \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{l}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{E}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{s}}\textcolor{black}{\textbf{\textless{}=}}$- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} / \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{l}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{E}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\textcolor{black}{\textbf{var(}}\textcolor{burntorange}{s}\textcolor{black}{\textbf{)}} / \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{c}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{E}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{s}}\textcolor{black}{\textbf{\textless{}=}}$- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{s}\textcolor{black}{\textbf{)}} \cdot \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{g} / \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{c}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{E}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{s}}\textcolor{black}{\textbf{\textless{}=}}$- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{s}\textcolor{black}{\textbf{)}} \cdot \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{r} / \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{l}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{E}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{InpV}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\frac{- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} + \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{fn}{\left(\textcolor{black}{\textbf{time}} \right)}}{\textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{r} \cdot \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{c}}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{E}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{InpV}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\left(- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} \cdot \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{r} + \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{fn}{\left(\textcolor{black}{\textbf{time}} \right)}\right) / \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{l}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{E}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{InpI}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{V}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\left(- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} \cdot \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{g} + \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{fn}{\left(\textcolor{black}{\textbf{time}} \right)}\right) / \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{c}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{prod(}}\textcolor{burntorange}{e}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{E}, \textcolor{burntorange}{s}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{InpI}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{-\textgreater{}}} \textcolor{burntorange}{t}\textcolor{black}{\textbf{:}}\textcolor{burntorange}{I}\textcolor{black}{\textbf{)}}
    \textcolor{black}{\textbf{t}}\textcolor{black}{\textbf{\textless{}=}}$\frac{- \textcolor{black}{\textbf{var(}}\textcolor{burntorange}{t}\textcolor{black}{\textbf{)}} + \textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{fn}{\left(\textcolor{black}{\textbf{time}} \right)}}{\textcolor{burntorange}{s}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{g} \cdot \textcolor{burntorange}{t}\textcolor{black}{\textbf{.}}\textcolor{burntorange}{l}}$\textcolor{black}{\textbf{;}}
  \textcolor{black}{\textbf{cstr}} \textcolor{burntorange}{V} \textcolor{black}{\textbf{\{}}
    \textcolor{ultraviolet}{\textbf{acc}}\textcolor{black}{\textbf{[}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{E}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{V}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{deepblue}{I}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{E}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{I}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{deepblue}{V}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{E}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{InpV}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{deepblue}{V}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{black}{\textbf{inf}}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{E}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{InpI}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{deepblue}{V}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{1}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{E}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{V}\textcolor{black}{\textbf{)}}
      \textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{\}}}
  \textcolor{black}{\textbf{cstr}} \textcolor{burntorange}{I} \textcolor{black}{\textbf{\{}}\textcolor{ultraviolet}{\textbf{acc}}\textcolor{black}{\textbf{[}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{E}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{I}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{deepblue}{V}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{E}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{V}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{InpV}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{InpI}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{deepblue}{I}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{1}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{E}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{I}\textcolor{black}{\textbf{)}}
      \textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{\}}}
  \textcolor{black}{\textbf{cstr}} \textcolor{burntorange}{InpV} \textcolor{black}{\textbf{\{}}\textcolor{ultraviolet}{\textbf{acc}}\textcolor{black}{\textbf{[}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{E}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{InpV}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{deepblue}{V}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{E}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{InpV}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{deepblue}{I}\textcolor{black}{\textbf{)}}
      \textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{\}}}
  \textcolor{black}{\textbf{cstr}} \textcolor{burntorange}{InpI} \textcolor{black}{\textbf{\{}}\textcolor{ultraviolet}{\textbf{acc}}\textcolor{black}{\textbf{[}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{E}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{InpI}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{deepblue}{V}\textcolor{black}{\textbf{)}}\textcolor{black}{\textbf{,}}
      \textcolor{ultraviolet}{\textbf{match}}\textcolor{black}{\textbf{(}}\textcolor{burntorange}{0}\textcolor{black}{\textbf{,}} \textcolor{burntorange}{1}\textcolor{black}{\textbf{,}}\textcolor{burntorange}{E}\textcolor{black}{\textbf{,}}\textcolor{deepblue}{InpI}\textcolor{black}{\textbf{-\textgreater{}}}\textcolor{deepblue}{I}\textcolor{black}{\textbf{)}}
      \textcolor{black}{\textbf{]}}\textcolor{black}{\textbf{\}}}
   \textcolor{black}{\textbf{\}}}
\end{Verbatim}
}

==> sections/introduction-scratch.tex <==


Domain specialists develop reconfigurable computations for their workloads in the agreed upon analog computing paradigm, and hardware designers extend the computing paradigm to capture different analog design points and limitations and model analog non-idealities. \tool{} deploys a programming language, called \toollang{}, that supports the specification of analog computing paradigms, and the specialization of these computing paradigms to codify analog design problems.


\todo{The following sections are placeholders. I'll continue to 1. check if any important ideas are missing 2. elaborate}
\subsection{Motivation}
\begin{itemize}
    \item The design and implementation of novel computing paradigms require expertise from multiple disciplines.
    \item Collaboration between domain experts and hardware designers is challenging due to their different perspectives.
    \item Require a \textbf{common abstraction} understood by both parties
    \item Utilize hardware designer's intents are important (Compared to digital, analog design has less well-defined models but relies on designer's intent... Cite the verification paper and the bag paper.)
    \item Enable DSE
    \item Why not conventional top-down flow? Analog automation/synthesis is hard, over-design, bottleneck in conversion, hard to do co-design (e.g., analog-to-information)
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/Ark System Overview - less text.pdf}
    \caption{Overview of the \tool{} system.}
    \label{fig:ark-overview}
\end{figure}

\section{\tool{} Design System}
\begin{itemize}
    \item \textbf{Language}
    The \tool{} specification language supports defining new types and dynamics of hardware elements and specifying constraints.
    Each specification contains type definitions, production rules, and validation rules. 
    \item \textbf{Compiler}
    \tool{} deploys a differential equation compiler to automatically generate a dynamical system that simulates the transient behavior of the hardware.
    \item \textbf{Validator} 
    \tool{} includes a verification procedure that checks if a given \model{} adheres to the specification to ensure that designs are physically plausible .
\end{itemize}

\proseheading{Domain Specialists' Tasks:}
\begin{itemize}
    \item Draft new designs
    \item Dynamical system simulation
    \item Design space exploration
    \item Negotiate over specification
\end{itemize}

\proseheading{Hardware Designers' Tasks:}
\begin{itemize}
    \item Provide initial specification
    \item Negotiate over specification
    \item Model more functions/ non-ideality if needed
    \item Implement in hardware
\end{itemize}


\subsection{Insights}
\begin{itemize}
    \item \textbf{Modeled with a system of ordinary differential equations (ODE)}. 
    The structure allows the system dynamics to be coupled to a graph representation.
    \item \textbf{Involve repeated sub-structures arranged in specific patterns}. 
    The graph is \textit{typed} and \tool{} is able to capture structural patterns with rules over graph components and their types.
    \item \textbf{Require iterative DSE across specialized domain and hardware}. 
    \tool{} enables practitioners to specify new types and rules that encompass crucial dynamics, such as functionality, design constraints, or non-idealities.
\end{itemize}

\proseheading{Broader Implications}

\newpage


==> sections/limitation.tex <==
\section{Limitation and Future Work}
\begin{itemize}
    \item No transient noise simulation support.
    \thoughts{
    We can hack a transient white noise simulation similar to what we did in \puf{} but can't guarantee efficiency or accuracy.
    From a practical perspective and the fact that transient noise simulation is very hard and performance-driven, I don't think implement it in \python make sense anyway.
    However, this is a reasonable/natural question to ask from a reviewer's perspective as noise is the most important non-ideality.
    One thing we can do is to state that noise simulation is delicate and that we should rely on dedicated tool for the task.
    Then, we show that we can map a circuit to a Spectre netlist, e.g., the \puf{} example.
    Also, we could point out that because the graph followed designer's intent, the mapping could be easier to write than in general.
    (Is it strong enough? 
    Also, another criticism might arise is that then domain specialist need to use the lower-level tool again.
    Perhaps another way to answer this question is to say that because noise is so unique that it belongs to lower-level modeling and we do/can not consider it in this level of abstraction (only the hacky solution if one really wants some noise simulation estimation)
    Technically we can implement stochastic differential equation integration in python with the Euler–Maruyama method and can use the package sdeint, the performance is still an issue though.
    }
\end{itemize}



==> sections/tech-implementation.tex <==
\section{Implementation}
\todo{Add citation}
The \tool{} type systems, compiler, and validator are implemented using the \python{} programming language. 
We utilize the built-in \textit{metaclass} feature provided by \python{} for custom typing and inheritance.
The compiler translate the dynamic graph into a system of differential equations, which is realized as a \python{} function. 
This function is designed to be compatible with the \textit{solve_ivp} function available in the \scipy{} package. 
The \textit{solve_ivp} function is then used to execute transient simulations.
The validator employs the Z3 SMT solver to solve the Integer Linear Programming (ILP) problem presented in the validation process.

==> sections/tech-lang-scratch.tex <==



\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\linewidth]{gen-figures/cdg/cdg-example.gv.pdf}
    \caption{Topology of $NT_i$ node. Intermediate edges omitted.}
    \label{fig:cdg-graph-formulation}
\end{figure}

\noindent\textbf{Deriving the Telegrapher's Equations.} The node type of the source node determines how terms are aggregated, and how the final relation is constructed. For example, the node type declaration \codein{node-type(1,sum) V} specifies that nodes of type \codein{V} sum up the terms contributed by connected edges, and the node dynamics are implemented with a first order (order=1) differential equation. For example, the node $V_1$ of type \codein{V} in the above dynamical graph implements the following differential equation:

\[
dV_1/dt = I_0/V_1.c - V_1/V_1.c - V_1/V_1.c \cdot V_1.g
\]

In the above equation, \codein{$V_1$.c} and \codein{$V_1$.g} to access the \codein{c} and \codein{g} attributes belonging to node \codein{V_1}, and each term is derived from a connection involving $V_1$. The \tool{}-derived differential equation matches the the differential equation for $dV_i/dt$ in the original telegrapher's equations math model.

\subsubsection{Reconfigurable Analog Circuits} 

Functions written in \tool{} design languages model reconfigurable analog hardware designs in the hardware design space. The function arguments define the programming interface of the reconfigurable hardware, and the body of the function instantiates the attributes, initial values, nodes, and edges that together model device parameters and the overall circuit topology. A subset of edges, initial values, and attributes are set by the function arguments. All other edges and attributes are set at fabrication time.


\section{Defining Reconfigurable Analog Computations with \tool{}-Lang}\label{sec:cdg:overview:speclan}

\begin{figure}
\subfloat[Grammar for \tool{} reconfigurable analog computations.]{
\parbox{\linewidth}{
\small
\begin{tabular}{lll}
% \multicolumn{3}{c}{$x \in \realnumbers$, $i,i',j \in \integers$, $b \in \booleans$, $v \in Literals$, $e \in Expressions$}\\
$GraphSt$ & ::= & \syn{node} $i$ : $v$ | \syn{edge}\syn{<} $i$\syn{,}$i'$ \syn{>} $j$: $v$ | \syn{switch} $i$\\
$Graph$ & ::= & \syn{analog-program} $v$ \syn{uses} $v'$ \syn{\{} $GraphStmt$* \syn{\}}\\
\end{tabular}
}
\label{fig:grammar:graph}
}\\
\subfloat[Grammar for configuring reconfigurable analog computations]{
\parbox{\linewidth}{
\small
\begin{tabular}{lll}

\end{tabular}
}
\label{fig:grammar:graphcfg}
}
\caption{\model{} graph language}
\end{figure}

Figure~\ref{fig:grammar:graph} presents the \model{} graph language. The graph language allows programmers to define a configurable, typed graph. The language defines  the following constructs.

\begin{itemize}[leftmargin=*]
\item The \codein{\syn{attr} v \syn{=} AVal} and \codein{\syn{attr} v \syn{=} ARng \syn{prog}} expressions instantiate a node or edge property \codein{v} to a constant \codein{AVal} or programmable \codein{ARng} value. Values may be booleans (\mathin{b}), integer valued (\mathin{i}), real-valued (\mathin{x}), or drawn from a real-valued distribution (\syn{N(}$x$\syn{,}$x'$\syn{)}). 

\item The \codein{\syn{initval} v \syn{=} ..} statements define the type of the initial value of stateful nodes to either a fixed (\codein{x}) or programmable value (\codein{[x,x'] \syn{prog}}). 

\item The \codein{\syn{node} i : v = Attr*} statements declares a node of type \codein{v} with an integer id \codein{i} and attribute values \codein{Attr*}. The \codein{\syn{switch} i'} defines a programmable switch with identifier \codein{i'}. The identifier \codein{i} uniquely identifies the node and switch in the graph.The programmable switches enable practitioners to design programmable topologies.

\item The \codein{\syn{edge} \syn{<}i\syn{,}i'\syn{>}: v = Attr*} statements declares a directed edge of type \mathin{v} with attribute values \codein{Attr*}.that connect nodes/switches \codein{i} to \codein{i'}. 
\end{itemize}

\subsection{Configuring Analog Computations}\label{sec:cdg:overview:configuration}


Figure~\ref{fig:grammar:graphcfg} presents the \tool{} graph configuration language. The graph configuration language lets end-users configure the programmable properties and withches in the \model{} graph:
\begin{itemize}[leftmargin=*]
\item{}The \codein{\syn{switch} i = i'} statements select the $i'$th edge at a programmable switch.
\item{}The \codein{\syn{node} i \syn{attr} v = AVal} statements instantiate a programmable property to the value \codein{AVal}. 
\end{itemize}
The \tool{} framework first \textit{configures} the configurable graph with a user-defined switch configuration and node and edge property configuration -- these configurations are used to eliminate programmable switches and concretize configurable edge and node properties.

\subsection{Configuring \subsubheading{\model{} Graphs}}
The \tool{} system applies the graph configuration to the \model{} graph specification to produce a \model{} graph that contains no switches or programmable parameters. The configuration procedure (\codein{\configurefn}) accepts a \model{} graph and a graph configuration and performs the following operation:

\begin{itemize}[leftmargin=*]
\item{}The \tool{} framework selects the appropriate edge for each switch, and then eliminates the switches from the graph by directly connecting each configured edge to the node downstream (or upstream) of the switch.

\item{}The \model{} framework applies the configuration to resolve all programmable attribute values to concrete numerical values, boolean values.

\item{} \tool{} samples stochastic parameters from their representative distributions and resolves these distributional parameters to constant values.
\end{itemize}
